Conormal Varieties on the Cominuscule Grassmannian - II

Let $X_w$ be a Schubert subvariety of a cominuscule Grassmannian $X$, and let $\mu:T^*X\rightarrow\mathcal N$ be the Springer map from the cotangent bundle of $X$ to the nilpotent cone $\mathcal N$. In this paper, we construct a resolution of singularities for the conormal variety $T^*_XX_w$ of $X_w$ in $X$. Further, for $X$ the usual or symplectic Grassmannian, we compute a system of equations defining $T^*_XX_w$ as a subvariety of the cotangent bundle $T^*X$ set-theoretically. This also yields a system of defining equations for the corresponding orbital varieties $\mu(T^*_XX_w)$. Inspired by the system of defining equations, we conjecture a type-independent equality, namely $T^*_XX_w=\pi^{-1}(X_w)\cap\mu^{-1}(\mu(T^*_XX_w))$. The set-theoretic version of this conjecture follows from this work and previous work for any cominuscule Grassmannian of type A, B, or C.

==> diagram2.tex <==
\begin{figure}[h]
\centering
\begin{center}
\begin{tikzpicture}[scale=.35]\footnotesize
 \pgfmathsetmacro{\xone}{0}
 \pgfmathsetmacro{\xtwo}{ 16}
 \pgfmathsetmacro{\yone}{0}
 \pgfmathsetmacro{\ytwo}{16}

\begin{scope}<+->;
 grid
  \draw[step=1cm,gray,very thin] (\xone,\yone) grid (\xtwo,\ytwo);

\end{scope}

\begin{scope}[thick,red]
  \foreach \x in {5,8,14,15,16}
    \draw (0, 16) rectangle (5,11);
    \draw (5, 11) rectangle (8,8);
    \draw (8, 8) rectangle (10,6);
    \draw (10, 6) rectangle (11,5);
    \draw (11, 5) rectangle (14,2);
    \draw (14, 2) rectangle (16,0);
% 
\draw[black] (2.5,13.5) node {\Large$ q_1$};
\draw[black] (6.5,9.5) node {\Large$ q_2$};
\draw[black] (9,7) node {\large$\bullet$};
\draw[black] (10.5,5.5) node {$\bullet$};
\draw[black] (12.5,3.5) node {\large$\bullet$};
%\draw[black] (9,7) node {\Large$\ddots$}
\draw[black] (15,1) node {\large$ q_l$};

\end{scope}
\end{tikzpicture}
\end{center}
\caption{Elements of $Q$}
\label{diagramtofu}
\end{figure}


==> old.tex <==

\begin{defn}
\label{defn:uw}
Let $R\define\left(\roots+..\backslash\roots.P.\right)\cap w^{-1}\left(\roots+..\right)$, i.e.,\begin{align*}
    R&=\set{\epsilon_i-\epsilon_j}{i\leq d<j,\,w(i)<w(j)}
\end{align*}
We define the vector subspace $\u_w$ of \u to be the sum of the root spaces corresponding to the roots in $R$, i.e., % basis \set{E_{i,j}}{w(i)<w(j)}.
\[
    \u_w\define\bigoplus\limits_{\epsilon_i-\epsilon_j\in R}[E_{i,j}]=\bigoplus\limits_{\substack{i\leq d<j\\ w(i)<w(j)}}[E_{i,j}]
\]
\end{defn}
The next proposition states that the \emph{generic fibre} of $\pi_w$ is isomorphic to $\u_w$.

\begin{prop}[cf. \cite{lakshmibai2017cotangent}]
\label{prop:uw}
The conormal variety \con\ is the closure in $T^* \nicefrac GP$ of\begin{equation*} 
    \left\{(bw,Y)\in G\times^P\u\mid\,b\in B,\,Y\in\u_w\right\}
\end{equation*}
\end{prop}

\subsection{The Subgroup $Q$}
Let $Q\define Stab_P(\u_w)$.
It follows from \Cref{b-stable} that $Q$ is a standard parabolic subgroup of $G$.
%\subsection{A Vector Bundle on $X_Q(w)$}
Consider the $G$-equivariant vector bundle $G\times^Q\u_w$ over $G/Q$. 
We have the following Cartesian square:\[
\begin{tikzcd}
    \rnw\arrow{d}\arrow{r}& G\times^Q\u_w\arrow[d]\\
    X_Q(w)\arrow[r]                                 & G/Q
\end{tikzcd}%\qquad\qquad
\]

\subsection{The Root System}
\label{rootSystemA}
Let $\mathfrak h$ be the set of diagonal matrices in $\mathfrak g$. 
For $1\leq i\leq n$, let $\epsilon_i\in\mathfrak h^*$ be given by \[
    \left\langle\epsilon_i,\sum\limits_{j=1}^n a_jE_{j,j}\right\rangle=a_i,
\]
where $E_{j,j}$ is the diagonal matrix with entry $1$ in the $j^{th}$ position and zero elsewhere.
The set of roots $\roots..$ of $\mathfrak g$ with respect to $(\mathfrak b,\mathfrak h)$ is precisely:\[
    \roots..=\left\{\epsilon_i-\epsilon_j\mid\,1\leq i\neq j\leq n\right\}
\]
We denote by $E_{i,j}$ the elementary $n\times n$ matrix with $1$ in the $(i,j)$ position and $0$ elsewhere; and by $[E_{i,j}]$ the one-dimensional subspace of \lgl\ spanned by $E_{i,j}$.
The root space corresponding to the root $\epsilon_i-\epsilon_j$ is precisely $[E_{i,j}]$.

\subsection{Simple Roots}
The roots $\alpha_i\define\epsilon_i-\epsilon_{i+1}$ are called \emph{simple} roots.
The set $S$ of simple roots forms a $\mathbb Z$-basis for \roots...
%Let $\preceq$ be the additive partial order on \roots.. gi
Let $\preceq$ be the partial order on \roots.. given by %:\begin{align*}
$    \epsilon_i-\epsilon_j\preceq\epsilon_k-\epsilon_l\text{ if and only if }i\geq k\text{ and }j\leq l$.
%\end{align*}
Equivalently, we have $\alpha\preceq\beta$ if and only if $\beta-\alpha$ is a positive linear combination of the simple roots $\alpha_i$.

\subsection{Minimal Representatives}
Let $\underline q=(q_1,\cdots,q_l)$ be a (weakly) increasing sequence with $0\leq q_i\leq n$. 
We say that $w\in S_n$ is \emph{minimal} with respect to $\underline q$ if for every $0\leq i\leq l$, we have $w(q_i+1)<w(q_i+2)\cdots<w(q_{i+1})$, where we set $q_0=0$ and $q_{l+1}=n$.

For $w\in S_n$, we denote by $w^{\underline q}$, the unique permutation achieved by rearranging in increasing order, for each $0\leq i\leq l-1$, the entries of $w$ in positions $q_i+1,q_i+2,\cdots, q_{i+1}$.
We will write $W^{\underline q}$ for the subset of $W$ comprising the elements which are minimal with respect to $\underline q$.
\subsection{Schubert Conditions}
For $V$ a subspace of \E n., we will say that $V$ satisfies the \emph{weak Schubert condition} $S_w(d)$ (or simply weak $S_w(d)$) if\begin{align}\label{weak}
    \dim(V\cap\E j.)\geq \mw (j,d)\qquad\forall\ j.
\end{align}
If $V$ further satisfies the condition $\dim V=d$, we say that $V$ satisfies the \emph{strong Schubert condition} $S_w(d)$ (or simply weak $S_w(d)$).
Observe that the statement `$V$ satisfies strong $S_w(d)$' is equivalent to the statement `$V\in X_d(w)$'. 

\begin{framed}
In this case, the map $\F\underline q.\mapsto F_d$ is precisely the birational map $\operatorname{pr}:X^Q_w\rightarrow X_w$ induced by the quotient map $\nicefrac GQ\rightarrow\nicefrac GP$. 

\begin{theorem}
\label{bir1}
It induces an isomorphism $X^\circ_{\underline q}(w)\rightarrow X^\circ_d(w)$ between the Bruhat cells; 
the inverse map $X^\circ_d(w)\rightarrow X_{\underline q}^\circ(w)$ needs to be better described.

is given by %\begin{align*}
    $F_d\mapsto (F_d\cap \E q_i.)_i$.
 %\end{align*}
\end{theorem}
\end{framed}

